Profiling Software Developers with Process Mining and N-Gram Language Models

Context: Profiling developers is challenging since many factors, such as their skills, experience, development environment and behaviors, may influence a detailed analysis and the delivery of coherent interpretations. Objective: We aim at profiling software developers by mining their software development process. To do so, we performed a controlled experiment where, in the realm of a Python programming contest, a group of developers had the same well-defined set of requirements specifications and a well-defined sprint schedule. Events were collected from the PyCharm IDE, and from the Mooshak automatic jury where subjects checked-in their code. Method: We used n-gram language models and text mining to characterize developers' profiles, and process mining algorithms to discover their overall workflows and extract the correspondent metrics for further evaluation. Results: Findings show that we can clearly characterize with a coherent rationale most developers, and distinguish the top performers from the ones with more challenging behaviors. This approach may lead ultimately to the creation of a catalog of software development process smells. Conclusions: The profile of a developer provides a software project manager a clue for the selection of appropriate tasks he/she should be assigned. With the increasing usage of low and no-code platforms, where coding is automatically generated from an upper abstraction layer, mining developer's actions in the development platforms is a promising approach to early detect not only behaviors but also assess project complexity and model effort.

==> appendices.tex <==

\appendix

%\noindent\textbf{Appendix A}
\section{Appendix}
\label{app:Appendix5}

\plot{chapter7-6.pdf}[Development fingerprints for the top(8) performers][13][ht!][trim=0cm 0cm 0cm 0cm]

\plot{chapter7-7.pdf}[Development fingerprints for the bottom(8) performers][13][ht!][trim=0cm 0cm 0cm 0cm]

\plot{chapter5-Top5.pdf}[Process Model characterizing Top5 Participants][14][ht!][trim=1cm 1cm 1cm 0cm]

\plot{chapter5-Bottom5.pdf}[Process Model characterizing Bottom5 Participants][14][ht!][trim=1cm 1cm 1cm 0cm]


%\subsection{Sub Topic}
